Patient-specific modelling, simulation and real-time processing for respiratory diseases

Asthma is a common chronic disease of the respiratory system causing significant disability and societal burden. It affects more than 300 million people worldwide, while more than 100 million people will likely have asthma by 2025. The price of asthma varies greatly from nation to nation. Mean yearly cost can be estimated to 1900 EUR in Europe and $3100 in the United States. Managing asthma involves controlling symptoms, preventing exacerbations, and maintaining lung function. Improved asthma control is reduces the risk of exacerbations and lung function impairment while reducing the direct costs of asthma care and indirect costs associated with reduced productivity. Understanding the complex dynamics of the pulmonary system and the lung's response to disease is fundamental to the advancement of Asthma treatment. Computational models of the respiratory system seek to provide a theoretical framework to understand the interaction between structure and function. Their application can improve pulmonary medicine by a patient-specific approach to medicinal methodologies optimizing the delivery given the personalized geometry and personalized ventilation patterns. A three-fold objective is addressed within this dissertation. The first part refers to the comprehension of pulmonary pathophysiology and the mechanics of Asthma and subsequently of constrictive pulmonary conditions in general. The second part refers to the design and implementation of tools that facilitate personalized medicine to improve delivery and effectiveness. Finally, the third part refers to the self-management of the condition, meaning that medical personnel and patients have access to tools and methods that allow the first party to easily track the course of the condition and the second party, i.e. the patient to easily self-manage it alleviating the significant burden from the health system.

==> figures/lstm/LSTMequations.tex <==
In these equations, $\mathrm{sigm}$ and $\tanh$ are applied element-wise. Figure \ref{fig:lstm} illustrates the LSTM equations.
\begin{figure}
  \begin{center}
    \begin{picture}(200, 130)
      \put(0, 0){\framebox(180, 100){}}
      \put(90, 50){\circle{16}}
      \put(86.5, 48){$\mathbf c_t$}
      \put(84, 60){{\scriptsize Cell}}
      \put(90, 32){\circle{6.5}}
      \put(87.25, 30.5){{\tiny $\times$}}
      \put(90, 12){\circle{16}}
      \put(86.5, 10){{\small $f$}}
      \put(100, 10){{\scriptsize Forget gate}}
      \put(90, 20){\vector(0, 0){8}}
      \put(85, 44){\vector(2, 3){0}}
      \qbezier(86, 32)(80, 36.5)(83, 41)
      \qbezier(96, 34)(100, 36.5)(95.5, 43.5)
      \put(93.5, 31.5){\vector(-1, -1){0}}
      \put(82, -8){\vector(1, 2){6}}
      \put(72.5, -13){{\small $h_{t-1}^{l}$}}
      \put(98, -8){\vector(-1, 2){6}}
      \put(99, -13){{\small $h_{t}^{l-1}$}}
      \put(30, 87){\circle{16}}
      \put(28, 85){{\small $i$}}
      \put(6, 85){{\scriptsize $\begin{matrix}\text{Input}\\\text{gate}\end{matrix}$}}
      \put(21.5, 105){\vector(1, -2){5}}
      \put(12.5, 108){{\small $h_{t-1}^{l}$}}
      \put(39.5, 107){\vector(-1, -2){6}}
      \put(37, 108){{\small $h_{t}^{l-1}$}}
      \put(147, 87){\circle{16}}
      \put(144.5, 85){{\small $o$}}
      \put(156, 85){{\scriptsize $\begin{matrix}\text{Output}\\\text{gate}\end{matrix}$}}
      \put(138.5, 105){\vector(1, -2){5}}
      \put(129.5, 108){{\small $h_{t-1}^{l}$}}
      \put(156.5, 107){\vector(-1, -2){6}}
      \put(154, 108){{\small $h_{t}^{l-1}$}}
      \put(17, 50){\circle{16}}
      \put(15, 48){{\small $g$}}
      \put(1, 28){{\scriptsize $\begin{matrix}\text{Input}\\\text{modulation}\\\text{gate}\end{matrix}$}}
      \put(53.5, 50){\circle{6.5}}
      \put(50.75, 48.5){{\tiny $\times$}}
      \put(57, 50){\vector(1, 0){25}}
      \put(25, 50){\vector(1, 0){25}}
      \put(35, 80){\vector(2, -3){17.5}}
      \put(147, 50){\circle{6.5}}
      \put(144.25, 48.5){{\tiny $\times$}}
      \put(98, 50){\vector(1, 0){45.25}}
      \put(150.5, 50){\vector(1, 0){38}}
      \put(147, 79){\vector(0, -1){25.5}}
      \put(190, 47){${\mathbf h^l_t}$}
      \put(-20, 40){{\small $h_{t-1}^{l}$}}
      \put(-20, 56){{\small $h_{t}^{l-1}$}}
      \put(-10, 44){\vector(4, 1){19}}
      \put(-10, 58){\vector(4, -1){19}}
    \end{picture}
  \end{center}
  \caption{A graphical representation of LSTM memory cells used in this paper (there are minor differences in comparison to Graves \cite{graves2013generating}).}
  \label{fig:lstm}
\end{figure}
